Goal-Driven Dynamics Learning via Bayesian Optimization

Real-world robots are becoming increasingly complex and commonly act in poorly understood environments where it is extremely challenging to model or learn their true dynamics. Therefore, it might be desirable to take a task-specific approach, wherein the focus is on explicitly learning the dynamics model which achieves the best control performance for the task at hand, rather than learning the true dynamics. In this work, we use Bayesian optimization in an active learning framework where a locally linear dynamics model is learned with the intent of maximizing the control performance, and used in conjunction with optimal control schemes to efficiently design a controller for a given task. This model is updated directly based on the performance observed in experiments on the physical system in an iterative manner until a desired performance is achieved. We demonstrate the efficacy of the proposed approach through simulations and real experiments on a quadrotor testbed.

==> notation.tex <==
% !TEX root = SysIdLQR.tex
\section{Notation and Preliminaries} \label{sec:notation}
In this section, we introduce two optimal control schemes, namely Model Predictive Control (MPC) and LQR, that will be used extensively throughout this paper.  

we formulate the controller design problem. Consider an unknown discrete-time, potentially non-linear, dynamical system:
\begin{equation} \label{eqn:sysmodel}
\state_{k+1} = \dyn(\state_k, \ctrl_k), k \in \{0, 1, \ldots, N-1\},
\end{equation}
where $\state_k \in \R^{n_x}$ denotes the system state and $\ctrl_k \in \R^{n_u}$ denotes the control input at time $k$. Given and initial state $\state_0$, the objective is to design a controller that minimizes the cost function $J(\state, \input)$. There are two main challenges in designing such a controller:
\begin{itemize}
\item how to model the unknown system dynamics in \eqref{eqn:sysmodel};
\item how to design the controller given this model.
\end{itemize}

In this work, we parametrize the unknown system in \eqref{eqn:sysmodel} as a time-invariant linear system. In other words, we aim to find a linearization of the system in \eqref{eqn:sysmodel} such that the controller designed to minimize $J$ for this linearized system also minimizes $J$ for the actual system. The effectiveness of this parametrization depends on both the system and the control objective. If $f$ is linear, then this parameterization is trivially sufficient for any control objective. When $f$ is non-linear, this parametrization may not be suitable for all control tasks; however, for regulation and trajectory tracking tasks, it is a common practice to linearize the system dynamics around the refernece set-point/trajectory and use the linearized dynamics to design the controller. Thus, for such tasks, a linear parameterization is often sufficient, as we also demonstarte in Section \ref{sec:numSim1}. A linear parameterization is also widely used in adaptive control \cite{sastry2011adaptive} framework.     



Even when the system dynamics are linear, it is not possible to design a controller for every $J$. We, thus, imnpose the following assumption on $J$:
\begin{assumption} \label{assump:cost}
The performance criterion, $J(x,u)$, is a convex function in $x$ and $u$.
\end{assumption} 
When $J$ is convex and dynamics are linear, we can use Model Predictive Control (MPC) scheme to efficiently design a controller that optimizes $J$ \cite{Camacho2013}. Given a linear system $\state_{k+1} = A\state_k + B\ctrl_k$ and a convex objective function $J$, MPC   



that penalizes the sys
\begin{equation} \label{eqn:cost}
J_N(\state_0) =\sum_{k=0}^{N-1}\left( (\state_k - \state^*)^T Q (\state_k - \state^*) + (\ctrl_k - \ctrl^*)^T R (\ctrl_k - \ctrl^*) \right) + (\state_N - \state^*)^T Q_f (\state_N - \state^*),
\end{equation} 

following the approach similar to \cite{Marco2016, trimpe2014self}. We start with a brief introduction of Linear quadratic regulator.

\subsection{Linear Quadratic Regulator (LQR)}
LQR is a well-known state feedback scheme for designing stabilizing controllers for steering a linear system to an equilibrium point. The technique can also be extended to nonlinear systems by linearizing the dynamics of the system about the equilibrium point. 

Consider a discrete-time non-linear dynamical system:
\begin{equation} \label{eqn:sysmodel}
\state_{k+1} = \dyn(\state_k, \ctrl_k),
\end{equation}
where $\state_k \in \R^{n_x}$ denotes the system state and $\ctrl_k \in \R^{n_u}$ denotes the control input at time $k$. Given a dynamically feasible reference state $\state^*$, and reference input $\ctrl^*$, the objective in LQR is to find a controller that minimizes the following quadratic cost starting from a given state $\state_0$,
\begin{equation} \label{eqn:cost}
J_N(\state_0) =\sum_{k=0}^{N-1}\left( (\state_k - \state^*)^T Q (\state_k - \state^*) + (\ctrl_k - \ctrl^*)^T R (\ctrl_k - \ctrl^*) \right) + (\state_N - \state^*)^T Q_f (\state_N - \state^*),
\end{equation}
\noindent where $Q$ and $R$ are positive definite matrices of appropriate size. For regulation problems such as steering a system to an equilibrium point, a linearized model around equilibrium is often sufficient for control design. Thus, we linearize \eqref{eqn:sysmodel} around $(\state^*, \ctrl^*)$. Defining the error dynamics $\bar{\state}_k = \state_k - \state^*$ and compensation input $\bar{\ctrl}_k = \ctrl_k - \ctrl^*$, the linearized system model can be written as:
\begin{align} \label{eq:err_dyn}
\bar{\state}_{k+1} =A\bar{\state}_k +B\bar{\ctrl}_k.
\end{align}
With respect to the linearized system, our goal is to design a controller that can keep the system at the equilibrium point $\bar{\state}_k = 0$ and $\bar{\ctrl}_k = 0$. Given the system matrices $(A, B)$ and the weights $(Q, R)$, the minimum cost to go $J^*_N$ can be solved recursively via dynamic programming, which also yields a time-invariant state feedback matrix $K$ that takes in the error state and outputs the appropriate compensation control. The closed loop control is thus given by
\begin{equation} \label{eqn:feedback_law}
\ctrl_k = \ctrl^* + K(\state_k - \state^*).
\end{equation} 
For simplicity, we write $K = LQR(A, B, Q, R, Q_f)$. 

Even though LQR controller can steer the system to an equilibrium point, the controller in \eqref{eqn:feedback_law} can be sub-optimal as it is designed for the linearized system and may not be optimal for the non-linear system in \eqref{eqn:sysmodel}. In such cases, automatic LQR tuning methods have been proposed in \cite{Marco2016, trimpe2014self}. But such an approach is sensitive to the accuracy with which the system matrices $(A, B)$ are known (for details see Section \ref{sec:comp1}). Moreover, when the system dynamics $\dyn(\cdot)$ in \eqref{eqn:sysmodel} are unknown or hard to model, it is not even possible to design an LQR controller. Thus, it might be desirable to learn the system matrices $(A, B)$ from the experimental data and then use \eqref{eqn:feedback_law} to design a stabilizing controller. This is the goal of the current work, which is detailed next. Note that one can also directly learn the feedback matrix $K$ when the system dynamics are unknown, as proposed in \cite{Calandra2015a}. There are some relative advantages and disadvantages of that approach over learning $(A,B)$ as discussed in Section \ref{sec:comp2}. 

\subsection{Control design problem}
We now consider the scenario where the system matrices $(A, B)$ are unknown. In this work, we parameterize the feedback gain $K$ in \eqref{eqn:feedback_law} as
\begin{equation} \label{eqn:Kparametrizn}
K(\theta) = LQR(A(\theta), B(\theta), Q, R, Q_f),
\end{equation}
where $A(\theta)$ and $B(\theta)$ are system matrices parameterized in $\theta \in \R^{D}$, which are to be varied in the learning procedure. When $\theta$ is varied, different matrix pairs $(A(\theta), B(\theta))$ (and thus different feedback matrices $K(\theta)$) are obtained. These feedback controllers will affect the system performance when applied to the actual system in \eqref{eqn:sysmodel} through \eqref{eqn:feedback_law}, thus resulting in a different cost value from \eqref{eqn:cost} in each experiment. To make the parameter dependence of \eqref{eqn:cost} explicit, we write
\begin{equation} \label{eqn:Costparametrizn}
J = J(K(\theta)) = J(\theta).
\end{equation}

The goal of the control design process is to vary the parameters $\theta$ such as to minimize the cost \eqref{eqn:cost}. Formally, the control design problem can be written as an optimization problem:
\begin{equation} \label{eqn:optzProb}
\argmin_{\theta} J(\theta) ~~\text{s.t.} ~~K(\theta) = LQR(A(\theta), B(\theta), Q, R, Q_f), \theta \in \thetaReg,
\end{equation}  
where we restrict the search of parameters to a bounded domain $\thetaReg \in \R^{D}$.    

The shape of the cost function in \eqref{eqn:optzProb} is unknown. Neither gradient information is available nor guarantees of convexity can be expected. The cost is thus evaluated empirically in each experiment. 
Such an evaluation is expensive as it involves conducting an experiment, which may last for a few minutes. 
Thus, the goal is to solve the optimization problem in \eqref{eqn:optzProb} with as fewer evaluations as possible.
In this paper, we do so through the use of Bayesian optimization, as described in the next section.



\SBnote{A few things to mention:
\begin{itemize}
\item Standard LQR problem is just a special case of regulation problem with the refernece point $(0,0)$.
\item Explain that trajectory tracking problem is also a regulation problem for a transformed non-linear system.
\item Explain motivation for choosing linear matrices even for non-linear system.
\end{itemize}}
